ShadowNet: A Secure and Efficient On-device Model Inference System for Convolutional Neural Networks

With the increased usage of AI accelerators on mobile and edge devices, on-device machine learning (ML) is gaining popularity. Thousands of proprietary ML models are being deployed today on billions of untrusted devices. This raises serious security concerns about model privacy. However, protecting model privacy without losing access to the untrusted AI accelerators is a challenging problem. In this paper, we present a novel on-device model inference system, ShadowNet. ShadowNet protects the model privacy with Trusted Execution Environment (TEE) while securely outsourcing the heavy linear layers of the model to the untrusted hardware accelerators. ShadowNet achieves this by transforming the weights of the linear layers before outsourcing them and restoring the results inside the TEE. The non-linear layers are also kept secure inside the TEE. ShadowNet's design ensures efficient transformation of the weights and the subsequent restoration of the results. We build a ShadowNet prototype based on TensorFlow Lite and evaluate it on five popular CNNs, namely, MobileNet, ResNet-44, MiniVGG, ResNet-404, and YOLOv4-tiny. Our evaluation shows that ShadowNet achieves strong security guarantees with reasonable performance, offering a practical solution for secure on-device model inference.

==> Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ *.log *.aux *.dvi *.bbl *.blg *.cb *.dep $(TARGET)

copy:
	cp paper.pdf $(HOME)/Desktop/modelsafe.pdf

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> RevisionLetter.tex <==
\clearpage
\title{\large\bf Revision Letter}

\newcounter{comment}
\newcommand{\comnote}{\arabic{comment}}

\newcommand{\concern}{\stepcounter{comment}\noindent\textcolor{red}{Concern \noindent\comnote }}
\newcommand{\response}{\noindent\textcolor{blue!50!black}{Response \noindent\comnote }}
\newcommand{\action}{\noindent \textcolor{green!50!black}{Action \noindent\comnote }}


\maketitle
This paper is a substantially improved re-submission of the paper \#344 from IEEE S\&P,  2022.
We would like to thank the reviewers for their detailed and thoughtful comments, which have inspired a number of changes and improvement to the paper. We have \textcolor{blue}{highlighted all the new text in  blue in the main paper} for the ease of reference.  Sec. \ref{rev:summary} outlines the main changes to the paper while in Sec. \ref{rev:comments}, we address each reviewer's comment individually. A PDF diff is attached at the end of the letter.
\section{Summary of Changes}\label{rev:summary}
We denote Review A as RA and so on.
The reviewer comments that are addressed by each of the itemized changes are stated inside the corresponding parenthesis. All the references in the revision letter to sections, figures, and tables refer to the revised submission.
%
\begin{enumerate}

\item \textbf{Larger and complicated models (Meta review and RB).} We have included evaluation results for two additional models, namely,  ResNet-404~\cite{he2016deep} and  Yolov4-tiny~\cite{YOLOPaper}. Both the models are significantly larger -- ResNet-404 is 28MB and YOLOv4-tiny is 33MB. Additionally, YOLOv4-tiny is the state-of-the-art object detection model which is a more complicated model.

\item \textbf{Reduce overhead (Meta review and RB).} We have proposed a new implementation optimization (Sec. \ref{sec:implementation:opt}) which has significantly improved our performance (Sec. \ref{sec:eval}). The current overhead for ShadowNet varies from $0.6\times$ to $1.6\times$  as opposed to $1.8\times$ to $3\times$ (for our previous submission). 


 
\item \textbf{Additional evaluation metrics (Meta review and RB).} We have included the consistency numbers in Fig. \ref{fig:accuracy}, Sec. \ref{sec:eval}. Additionally, we have retrained all our models to
match the corresponding state-of-the-art accuracies.


\item \textbf{Evaluate black-box attacks (Meta review and RD).}
We have added new experiments and additional details on black-box attacks in Sec. \ref{sec:sec_ana}.

\item \textbf{LSTM (Meta review and RB).} We have added an illustration of ShadowNet's support for LSTMs in Sec. \ref{sec:discussion}. 

\item \textbf{Object detection model (Meta review and RB).} We have added evaluation results for YOLOv4-tiny~\cite{YOLOPaper}, the state-of-the-art object detection model. 
\item \textbf{Details on proofs (Meta review and RB).} We have added the detailed clarification regarding the role of the obfuscation ratio $r$ in the secuirty proof in Sec. \ref{sec:sec_ana}. 
\item \textbf{Running unmodified model inside the TEE (RA, RB, RD).} We have added a discussion on why running the unmodified model inside the TEE is challenging in Sec. \ref{sec:discussion}.
\item \textbf{Title change (RB).} We have changed the title of the paper.

%\item \textbf{Comparison with other similar works (RB).} We have included a discussion in Sec. \ref{sec:related_work} on why comparison with other works is not feasible.
%\item \textbf{Modifiying TensorFlow (RC).} We have added a discussion in Sec. \ref{sec:TF} on why integrating ShadowNet into Tensorflow-Lite makes it easier for real-world usage.
\item \textbf{Details on quantization (RA, RC).} We have added details on the necessity of the quantization layer and its parameter values in Secs \ref{sec:sec_ana} and \ref{sec:implementation}.
\item \textbf{Writing improvement (RB).} We have fixed all the writing issues including restructuring several sections.
\end{enumerate}


\section{Reviewer Comments}\label{rev:comments}
%We now directly address reviewer‚Äôs comments,
%
When directly quoting reviewers comments, we will be using \textit{italic type font}. First we address the meta reviews followed by the individual comments from each reviewer.

\subsection{Meta Review Comments}\label{rev:MR}
\textcolor{white}{H}\\\\\noindent\textcolor{red}{Concern 1.} \textit{It is still unclear if ShadowNet can deal with other apps that use more complicated and larger models. The paper should evaluate with more complicated and larger models.}\\\\
\textcolor{blue}{Response 1.} We have added evaluations results for \textit{two} new larger and complex models in Sec. \ref{sec:eval}:
\begin{itemize}\item ResNet-404~\cite{he2016deep} of size $28$MB \item YOLOv4-tiny~\cite{YOLOPaper} of size $34$MB \end{itemize} 
ResNet models use shortcut connections between the
convolutional layers which create branches and merges in the network structure. ResNet-404 has size 28MB is which is significantly larger than the previously evaluated ResNet-44 (size 2.4MB). The ShadowNet overhead for ResNet-404 is 281 ms (1.5$\times$; Fig. \ref{fig:sn-perf}).


YOLOv4-tiny is a state-of-the-art object detection model for mobile devices and a more complex model. First, object detection requires a multi-task model/multi-objective optimization which outputs a prediction class and a bounding box. Second, the model structure itself is non-sequential with new activation operations, such as LeakyRelu~\cite{DBLP:journals/corr/RedmonDGF15}, and complicated Lambda layers consisting of different non-linear operations, such as upsampling, concatenation. Third, the original model size is 34MB which is large in the context of mobile environments. The ShadowNet overhead for YOLOv4-tiny is 451ms (0.7 $\times$; Fig. \ref{fig:sn-perf}). 


Additionally, we present a discussion on assessing how large a model can ShadowNet support as follows.  We start by analyzing the spatial overhead of ShadowNet.
\begin{table}[!ht]
\centering
\caption{ShadowNet model size change.}
\label{tab:sd-size}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
    \multicolumn{2}{c|}{Model Size(MB)} & MobileNet & ResNet-44 & ResNet-404 & YOLOv4-tiny & MiniVGG \\
    \hline
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Original\\ Model\end{tabular}} &   \textit{Conv} & 17 & 2.43 & 24.71 & 22.56 & 20 
    \\\cline{2-7} & \textit{Other} & 0.175 &0.029 & {0.23} & {0.79} &  0  \\ 
    \hline
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ShadowNet\\ Model \end{tabular}} & \textit{Conv} & 20& 2.92 &   29.79   & 27.11 &24  
    \\\cline{2-7} & \textit{Other} & 37 &3.3 &29.73  & 40.53 & 2  \\
\hline
\end{tabular} \vspace{-2mm}
}
\footnotesize
    {
        \\Model weights are divided into two parts -- \textit{Conv} layers' weights (standard convolutional, pointwise convolutional,
    depthwise convolutional and fully connected layers) and \textit{Other} layers' weights (\textit{AddMask}, \textit{LinearTransform}, \textit{ShuffleChannel}, \textit{Batchnorm}).
    Among the \textit{Other} layers, the weights of the \textit{AddMask} layer occupy the maximum space for ShadowNet models.} 
\end{table}

The above table shows the model size before and after the ShadowNet transformation. In general, ShadowNet can be applied to any CNN model as long as the TEE can support the memory requirements of the corresponding ShadowNet transformed model. The amount of TEE memory required for running the ShadowNet transformed model can be estimated by the size of the weights that need to be stored inside the TEE (see \textit{Other} in table above). Concretely, the total size is given by the sum of the size of the weights of four ShadowNet operations, namely, \textit{LinearTransform}, \textit{ShuffleChannel}, \textit{AddMask} and \textit{Batchnorm} (Sec. \ref{sec:implementation:conversion}).  The size of \textit{LinearTransform} and \textit{ShuffleChannel} can be computed from the shapes of the convolutional layer and the obfuscation ratio (Sec. \ref{sec:scheme}). The size of \textit{AddMask} can be computed from the input and output shape of each layer. The size of \textit{Batchnorm} can be computed directly from the model. 
%In general, ShadowNet can be applied to any CNN model as long as the TEE can support the memory requirements of the corresponding ShadowNet transformed model. The amount of TEE memory required for running the ShadowNet transformed model can be estimated by the size of the weights that need to be stored inside the TEE (see ``Other" in Table \ref{tab:sd-size} which shows the model sizes before and after ShadowNet transformation) which depends on the following two factors. First, it depends on the size of the transformed convolutional layers' weights which can be computed from the shape of the convolutional layers and the obfuscation ratio. Second, it depends on the weights of the mask layers which can be computed from the input and output shape of each layer. %As shown in Table \ref{tab:sd-size}, even though the original model can be big, the weights need to be stored inside TEE can be small (e.g., MiniVGG) or big (e.g., MobileNets). 
%Note that the actual runtime memory allocation required by ShadowNet is lesser due to our optimized memory allocation (Sec. \ref{sec:ca-ta}).  
We have added this discussion in Sec. \ref{sec:discussion} and Table \ref{tab:sd-size}.
\\\\
\noindent\textcolor{red}{Concern 2} \textit{ The current overhead is high. It is better to further reduce the overhead.}\\
\textcolor{blue}{Response 2 } We have proposed a new optimization for this revised submission that has improved ShadowNet's performance significantly (Tab. \ref{tab:perf-opt}). Recall that ShadowNet runs the transformed  linear (convolutional) layers  in the Normal World (untrusted CPU/GPU) and runs all the non-linear layers in the Secure World (TEE; see Fig. \ref{fig:system}). ShadowNet uses a client application (CA) in the Normal World to communicate with a trusted application (TA) in the Secure World. Our new optimization is aimed at reducing this communication cost between the CA and the TA and is detailed below.


\begin{table}[ht]
\centering
\caption{Impact of New Optimization}
\label{tab:perf-opt}

\begin{tabular}{lcc}
\hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{ShadowNet Overhead (ms)} \\
    & Current & Previous \\
\hline
MobileNets & $252 (1.6\times)$ & $468 (3\times)$\\
ResNet-44 & $30 (1.1\times)$ & $76(2.9\times)$ \\
MiniVGG & $5 (0.6\times)$ & $15 (1.8\times)$\\
ResNet-404 & $281 (1.5\times)$ & N/A\\
YOLOv4-tiny & $451 (0.7\times)$ & N/A\\

\hline
\end{tabular}

\end{table}

The OP-TEE OS is designed to work with a TA with a relatively small TEE memory usage ($<$1MB). 
As a result, for every call the CA makes to the TA, the TEE OS sets up a page mapping for the entire memory used by the TA even when the CA and the TA are in the same session. This has an adverse effect on the performance -- when the TA's memory size increases, the associated cost of the CA's call to the TA increases proportionately even when the TA is idle inside the TEE. For example, the time increase from 0.1ms to 6ms for a memory increase of 1MB to 64MB. This TEE design limitation is known to be a major challenge in the general OP-TEE community~\cite{optee-issue1,optee-issue2}. In order to tackle this, we propose a novel optimization as follows. Note that only the parameters (handles for the memory shared between the CA and the TA) of the CA's call change  and require a new mapping every time -- the majority of the TA's memory, namely the data and code, do not need to be re-mapped for every call. Based on this observation, we implemented an optimization in the TEE OS to cache the page mapping for the TA's code and data section. Only the pages corresponding to the parameters passed between the CA and the TA are re-mapped. This improves the performance significantly -- the results are depicted in Table \ref{tab:perf-opt}; column 1 shows the overhead of the current (revised) submission while column 2 shows the overhead of our previous submission. For instance for MiniVGG, the ShadowNet overhead reduces from $15$ms to $5$ms -- a $3\times$ improvement.  %For instance for MobileNets, the total model inference time on CPU decreases by 35\%, from 643ms to 407ms.
Since the memory limitation of the TA is a well-known challenge in the OP-TEE community, we believe that our key idea of caching certain pages could be of independent interest to the broader OP-TEE community.
\\\\\textcolor{red}{Concern 3 } \textit{ Additional evaluation metrics. The evaluation should report on the consistency. When you protect more layers, you may need to record the changes of consistency. In addition, the accuracy of the models should be improved to a comparable accuracy with other state-of-the-art works.}
\\\textcolor{blue}{Response 3 }  We have included the consistency numbers in Fig. \ref{fig:accuracy} in Sec. \ref{sec:eval}. Specifically, ShadowNet's Top1 prediction consistency for ResNet-44, ResNet-404, MiniVGG, YOLOv4-tiny and MobileNet are $97\%$, $96\%$, $98\%$, $94\%$ and $88\%$, respectively. The relatively low consistency for MobileNet is due to the inputs which are predicted \textit{incorrectly} by the original model. Specifically for inputs with correct predictions from the original model, ShadowNet is $95\%$ consistent; for the incorrect predictions, ShadowNet is $74\%$ consistent. The original model's mean confidence (top-1 score) for the inputs with correct and incorrect prediction is $0.8$ and $0.38$, respectively. Recall that MobileNet is evaluated on ImageNet with 1K classes. Hence for classification tasks with such a large number of classes, ShadowNet's numeric errors can impact inputs that have \textit{low confidence scores} from the original model (for instance, the top-2 scores are very close). The performance is acceptable since this affects mostly the inputs with \textit{incorrect} predictions from the original model. 
\par We have retrained all the models to match their corresponding state-of-the-art accuracies (Fig. \ref{fig:accuracy}).  
\\\\
%\textcolor{red}{Concern 2.} \textit{Similarly, consider ways to reduce the overhead.}
%\textcolor{blue}{Response 2.}\todo We have 
%\\\\
\\\\\textcolor{red}{Concern 4. }  Evaluate black-box attacks and provide more details.\\
\textcolor{blue}{Response 4. }  The threat model of ShadowNet assumes that the adversary has access to the model's querying API, i.e.,  $Y=\mathcal{M}(X)$\footnote{some extra information about the architecture, such as the number and type of linear layers, is also allowed -- see Sec. \ref{sec:sec_ana} for details)}. Hence, based on our formal security guarantee (Thm. \ref{thm:1}), we present the following conjecture:
\point{Conjecture 1} \textit{Let $q$ be the number of queries required for a  model stealing attack with access to just the querying API, i.e., $Y=\mathcal{M}(X)$ (black-box model stealing attack) and some information about the model architecture (such as, number and type of convolutional layers). Let $q'$ be the number of queries required for an attack on  ShadowNet. We conjecture that $q'$ is of the order of $O(q)$.}
\\\\
Black-box model stealing attacks can be typically classified into two types:
\begin{itemize} \item Functionally-equivalent model stealing attacks \cite{jagielski2019high} where the attacker tries to extract the \textit{exact} weights of model by analytically solving a set of linear equations.
\item  Learning-based model stealing attacks where the adversary tries to learn a shadow model \cite{tramer2016stealing,Knockoff,MixMatch}. 
\end{itemize}
The first type of attacks are impossible in ShadowNet -- since our mask layers are refreshed every time, it is mathematically impossible to solve for the model weights (Lemma \ref{lemma:1}, App. \ref{app:sec_ana}). 

Clearly from our threat model (Sec. \ref{sec:threat}), protection against learning-based black-box model stealing attacks is \textit{beyond the scope} of ShadowNet. The implications of Conjecture 1 in this context is that with ShadowNet, an adversary cannot do anything significantly better than a standard learning-based black-box model stealing attack. %In other words, an adversary cannot learn anything useful about the original weights by observing the ShadowNet transformed weights. 
In what follows, we present empirical evidence for the above conjecture. To reiterate, the goal of our analysis is to show that ShadowNet provides \textit{no extra advantage} to an adversary carrying out standard black-box model stealing attacks. %We provide new empirical evidence (Tab. \ref{tab:BB}) in support of our conjecture in Sec. \ref{sec:sec_ana}. 
%We reproduce the results below for the ease of reading.  
\\\\\textcolor{red}{Concern 4a. } \textit{ What kind of black-box attack are you using?}\\
\textcolor{blue}{Response 4a. } We evaluate two state-of-the-art black-box attacks, namely, MixMatch~\cite{MixMatch,jagielski2019high} and Knockoff~\cite{Knockoff}. We chose these attacks since a recent survey~\cite{pow2022iclr} shows that MixMatch is currently the state-of-the-art attack with the \textit{highest} attack accuracy. On the other hand, Knockoff is the state-of-the-art black-box attack with an \textit{adaptive} query strategy. The  victim model is a four layer fully-connected CNN trained on CIFAR-10 as shown in Fig. \ref{fig:example-cnn}. \\\\
\textcolor{red}{Concern 4b. } \textit{How to choose the dataset for querying? How many queries are needed to attack ShadowNet?} \\
\textcolor{blue}{Response 4b. } We have explored two different querying strategies with our evaluated attacks. The MixMatch attack samples 8K points from CIFAR-10 for querying the victim model and uses an additional 8K unlabeled points from CIFAR-10 for its semi-supervised training. 
Knockoff queries the victim model from an out-of-distribution dataset. For our evaluation,  Knockoff uses 10K queries from CIFAR-100~\cite{cifar100} selected via an adaptive strategy based on reinforcement learning.  \\\\
\textcolor{red}{Concern 4c. }\textit{What is the benefit of an attacker having $\hat{W}$ compared to having no knowledge of the model?}\\
 \textcolor{blue}{Response 4c. }
  
 \begin{table}[!ht] 
\centering
\caption*{Empirical evaluation of black-box attack}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c}\hline
Black-box Attack &Victim & Attack Baseline & ShadowNet & Random Baseline  \\\hline
% we don't have consistency data for MixMatch
%\new{Consistency}&\new{40.1\%} & \new{33.1\%}& \new{38.4\%} \\
Knockoff~\cite{Knockoff} & 81.6\%& 36.6\% & 31.1\% & 36.2\%  \\
MixMatch~\cite{MixMatch,jagielski2019high} & 98.1\% & 95.8\% & 92.3\% & 92.4\%  \\
\hline
\end{tabular}}
   \vspace{-2mm}
\end{table}
The results of our evaluation is presented in the above table. The  victim model is a four layer fully-connected CNN as shown in Fig. \ref{fig:example-cnn}. For Knockoff, the victim model is trained on CIFAR-10 with accuracy 81.6\% (column 1). For MixMatch, the victim model is trained on CIFAR-10 with the MixMatch semi-supervised training approach and has accuracy 98.1\% (column 1). We used different training strategies for the victim model for the two attacks in order to be consistent with the configurations of their respective original papers~\cite{Pow_repo}. The baseline shadow model (column 2) for Knockoff and MixMatch is  ResNet-18 and Wide-ResNet-28, respectively -- this corresponds to the attack baseline with no knowledge of the victim model. %All the attack hyperparameters and setting configurations are kept the same as in the original papers for both the attacks~\cite{Pow_repo}. 

In order to assess whether the adversary benefits from knowing the transformed weights ($\hat{W}$) in ShadowNet, $(1)$ we create a custom adversary model  with the same architecture as that of the victim, $(2)$ we copy the
 weights $\hat{W}$ to the adversary’s model, (3)  we mark the convolutional layers with weights $\hat{W}$  as non-trainable and
train only the other layers (results in column 3). The resulting adversary model is depicted in Fig. \ref{fig:attacker_net} in App. \ref{app:sec_ana}. Thus, column 3 corresponds to the attack setting adapted for ShadowNet where the adversary has access to the victim model's transformed weights. We observe that the ShadowNet adapted attack is less accurate than the baseline attack (column 2) after the same number of queries. In fact,  the ShadowNet adapted attack performs worse than a random baseline (column 4) where the weights of the non-trainable convolutional layers (as described above) are randomly assigned.  This shows that the ShadowNet transformed weights contain no useful information about the original weights and the adversary gains \textit{no advantage} by reusing the transformed weights.
%In column 4, we measure a random baseline  This shows that the ShadowNet transformed weights contain no useful information about the original weights and the adversary gains no advantage by reusing the transformed weights. %-- this corresponds to the case where the attacker has access \textit{only} to the victim model architecture (no transformed weights). 

  %The random baseline (column 4) also performs worse than the attack baseline (column 1) which shows that victim model architecture information is not useful for the attack either.


    %In order to assess whether the adversary benefits from knowing the transformed weights (conv') in ShadowNet, (1) we create a customized adversary model with the same architecture as that of the victim model, (2) we copy theconv’ layers to the adversary’s model, (3)  we mark these conv’ layers as non-trainable and onlytrain the other layers (results in column 2). For the Random Baseline attack,  the weights of the non-trainable convolutional layers are randomly initialized. } 
 
 
 All of the above discussion is included in Sec. \ref{sec:sec_ana}. 
\\\\\textcolor{red}{Concern 5. } \textit{Similarly, while the paper says that it can handle model layers of different types, such as LSTM, the authors do not evaluate any models that use them. If the paper provides a small example of it working for object recognition, audio recognition, etc., it will make the paper more convincing.}
\\
\textcolor{blue}{Response 5. } We have added evaluation results for YOLOv4-tiny in Sec. \ref{sec:eval} which is the state-of-the-art object detection model that is more complex than a regular CNN (see our response to Concern 1 earlier for more details). 

LSTM's are the state-of-the-art models used for speech recognition. We provide an illustration of ShadowNet's support for LSTMs as follows.  
  \begin{figure}[ht]
   \centering
   \includegraphics[width=0.8\linewidth]{figs/LSTM-Shadownet-2.pdf}\vspace{-2mm}
     \caption*{\textbf{Illustration of ShadowNet transformation on LSTM}}. 
 \end{figure}
 LSTMs typically consist of fully-connected layers, pointwise matrix operations and activation layers. Recall that a fully connected layer can
     be treated as a convolutional layer during ShadowNet transformation. Hence for LSTMs, ShadowNet applies linear transformation on the fully connected layers while keeping the pointwise matrix operations and activation layers inside the TEE. 
     
     As a concrete example, a LSTM layer (top)  and its corresponding ShadowNet transformation (bottom) is depicted in the figure above.  %We implemented a prototype ShadowNet transformation for the LSTM layer depicted above with an input ($x_t$) shape  of $(10, 30)$, output space/units set to be $10$, $1640$ parameters and obfuscation ration $r=1.2$.  The ShadowNet transformed layer has the same input and output shape as the original LSTM layer and can seamlessly replace it. %Inside it, it uses PushMask, LinearTransform and PopMask "PUSHM", "CONV'","LT",  "POPM" operations to replace original fully connected layer . We observe that the number of parameters after the ShadowNet transformation is $3640$ -- the extra parameters are due to the mask layers and the transformed CONV$'$ layers. 
  %When we set obfuscation ratio as $1.2$, it has 3640 parameters. The extra parameters come from the mask layers and the transformed "CONV'" layers.
 The red circles represent pointwise matrix operations and the yellow square boxes marked with activation symbols represent
    fully connected layers followed by the corresponding activation layers.   Green boxes marked ``LT", ``PUSHM" and ``POPM" represent  the ``LinearTransform", ``PushMask" and ``PopMask" layer of ShadowNet, respectively (same as the ones in Sec. \ref{sec:implementation}). The yellow square boxes marked with ``CONV$'$" represent the ShadowNet transformed convolutional layers
     which are computationally heavy and can be outsourced to the untrusted world for acceleration. 
     All the other parts of the LSTM layer including the internal states remain in the Secure World. 
     
  We implemented a prototype ShadowNet transformation for the LSTM layer depicted above with an input ($x_t$) shape  of $(10, 30)$, output space/units set to be $10$, obfuscation ration $r=1.2$ and $1640$ model parameters.  The ShadowNet transformed layer has the same input and output shape as the original LSTM layer and can seamlessly replace it. We observe that the number of parameters after the ShadowNet transformation is $3640$ -- the extra parameters are due to the mask layers and the transformed CONV$'$ layers. The above discussion is included in Sec. \ref{sec:discussion}. %Inside it, it uses "PUSHM", "CONV'","LT",  "POPM" operations to replace original FullyConnect layer. 
  %When we set obfuscation ratio as $1.2$, it has 3640 parameters. The extra parameters come from the mask layers and the transformed "CONV'" layers.

 

Here we would like to stress that the focus of ShadowNet is convolutional neural networks (CNN). We have also changed our title to "ShadowNet: A Secure and Efficient
 On-device Model Inference System for \textcolor{blue}{Convolutional Neural Networks}" to highlight this. The purpose of the discussion above is just to demonstrate the feasibility of applying ShadowNet to architectures beyond CNNs. A full-fledged exploration of other architectures is a part of future work.
\\\\\textcolor{red}{Concern 6.} \textit{The additional explanation on proofs is valuable and it makes sense. These detailed clarifications must be provided in the paper, it would be helpful for readers to understand your design consideration.}\\\textcolor{blue}{Response 6.} We have added the detailed clarification in Sec. \ref{sec:sec_ana} and reproduce it here for the ease of reading.

Intuitively, the parameter $r$ is analogous to the security parameter (such as, key size) for generic cryptographic protocols. The larger the value of the obfuscation ratio $r$, the greater is the size of the feasible set and consequently, the better is the security. Concretely, $\mathcal{F}(\hat{W}_a)\supset \mathcal{F}(\hat{W}_b)$ where $m_a=|\hat{W}_a|>|\hat{W}_b|=m_b$ (equivalently, $r_a>r_b$). $r$ is essentially a trade-off between the security guarantee and performance. The exact size of feasible sets can be analytically computed (see App. \ref{app:sec_ana}). Fig. \ref{fig:obf_ratio} shows ShadowNet’s performance with varying values of $r$. Based on this, we set $r=1.2$ for our experimental setup since this was the sweet spot. Specifically, even with $n=16$ (smallest $n$ for our evaluation) and field $\mathbb{F}=\mathbb{Z}_p$
  for $p=2^{24}-3$, the size of the feasible set, $|\mathcal{F}(\hat{W})|$, is of the order of $2^{268}$
  which is sufficient for security. The reason why we get a large feasible set even with a relatively small value of $r$ is that the random permutation matrix $P_\pi$
  and random scalar multiplications by $\lambda_i$s also contribute significantly to the size of the feasible set.

\subsection{Review A}
\textcolor{white}{H}\\
\textcolor{red}{Concern 1. }\textit{It would be informative to also provide a comparison with the unmodified model running entirely in the TEE. 
...
It seems like running ShadowNet would increase the TCB more than running the unmodified model, because of the additional complexity introduced to obfuscate the layers and mask the intermediate inputs.
}\\\textcolor{blue}{Response 1. } There are several challenges in running the unmodified model inside the TEE. First, standard model inference (outside the TEE) is memory intensive. For instance, convolution operations are expensive as they require resizing of the dimensions of the matrices. Additionally, buffers are allocated dynamically to store the intermediate results for the output of each layer.  Our memory profiling shows that running the unmodified model inference requires dynamically allocating at least 44MB for MiniVGG, 10MB for ResNet-44, 61MB for MobileNet, 54MB for ResNet-404 and 72MB for YOLOv4-tiny. Also note that the secure OS inside the TEE reserves $>$4MB memory for its usage. Hence given the TEE memory limit of $64$ MB for our evaluation board, it is not feasible to run the entire model inference task inside the TEE. ShadowNet, on the other hand, only requires 4MB for MiniVGG, 5MB for ResNet-44, 48MB for MobileNet, $34$MB for ResNet-404 and $52$MB for YOLOv4-tiny, thereby requiring a much smaller secure memory size. 

Second, running unmodified models inside the TEE would require a significant engineering effort. TensorFlow Lite needs to be ported into the TEE for the convolutional layers and matrix operations which rely on certain mathematical libraries (in C++) for efficiency. This entails a significant engineering effort since currently Arm OP-TEE OS does not support C++ and its corresponding computing libraries.  

Third, the limited size of the TCB presents additional challenges. A core focus of ShadowNet's design and implementation optimizations was to make it work with a small TCB -- its TA adds only 2100 LOC inside the TEE. Specifically, the new operations introduced by ShadowNet (LinearTransform, AddMask, ShuffleChannel) add $<$200 LOC into TCB as they are relatively simple operations.  On the other hand, TensorFlow Lite has tens of thousands lines of code and porting it as a whole inside TEE would require a much larger TCB. ShadowNet, by design, keeps it outside the TCB, thereby allowing a user to enjoy its rich functionality in a secure manner with a small TCB. Additionally, note that the extra code added for model conversion is used offline by the model vendor and is not deployed on the device. Hence, this does not increase the device TCB size.

Last, we will lose access to hardware accelerators if we run the unmodified model inside the TEE. We have included the discussion in Secs.  \ref{sec:scheme_opt}, \ref{sec:implementation} and \ref{sec:discussion}.
\\\\
%\textcolor{red}{Concern 2. } \textit{}\\
%\textcolor{blue}{Response 2. } Shadownet’s TA inside the TEE adds only 2100 LOC.  Note that TensorFlow Lite has tens of thousands lines of code and porting it as a whole inside TEE would require a much larger TCB.  Additionally, note that the extra code added for model conversion is used offline by the model vendor and is not deployed on the device. Hence, this does not increase the device TCB size. We have included this discussion in Sec. \ref{sec:scheme_opt} and \ref{sec:implementation}.
%\\\\
\textcolor{red}{Concern 2. }\textit{The paper also makes the argument that some model sizes exceed the memory available to the TEE. However, this doesn't take into account whether the entire model needs to be loaded at once, or whether e.g. the layers could be loaded sequentially to remain within memory constraints.}
\\
\textcolor{blue}{Response 2. } The suggestion of loading the model layer by layer would indeed save memory. However, this would require reloading the model weights for each round of model inference which would be costly in terms of runtime -- this is partly reflected in the time required for refreshing the mask weights (one of the costliest steps in ShadowNet).
\\\\\textcolor{red}{Concern 3. }\textit{It would be helpful to also quantify the computational overhead of these pre-computation steps (separately from the online performance evaluation).}\\
\textcolor{blue}{Response 3. }
Offline model conversion takes $10$min $59$s for MiniVGG, $6$min 5s for ResNet-44, $31$min $23$s for MobileNet, $28$min $46$s for ResNet-404, $24$min $23$s for YOLOv4-tiny. Regeneration of mask layers' weights for $100$ instances takes $2.19$s for MiniVGG, $20.29$s for ResNet-44, $97.26$s for MobileNet. $127.9$s for ResNet-404, $25.5$s for YOLOv4-tiny. We have included the details in Sec. \ref{sec:efficiency}.
\\\\
\textcolor{red}{Concern 4. }\textit{It wasn't clear from the paper why the weights had to be quantized and de-quantized. This could be explained in more detail in the paper.}\\
\textcolor{blue}{Response 4. } The quantization is required for providing a formal security guarantee for the mask layer and the reason is explained as follows. The quantization operation embeds the value in a finite field, $\mathbb{F}$. Subsequently, the masks can be chosen uniformly at random from $\mathbb{F}$ thereby making the mask layer equivalent to one-time-pad encryption \cite{KatzLindell}. Without quantization, we would have to deal with real numbers (floating points) – we cannot give any formal security guarantee here since there exists no uniform distribution over reals. The values are de-quantized inside the TEE for computing the non-linear layers.
We have included the details in Sec. \ref{sec:sec_ana}.\\\\
\textcolor{red}{Concern 5. }\textit{Did you consider using a ``switchless" approach where specific threads/cores remain in the secure world and communicate with the Normal World using shared memory?}\\\textcolor{blue}{Response 5. }  
We have implemented a new optimization for reducing the communication cost between the Normal World and the Secure World that has significantly improved ShadowNet's performance (see Concern 2 in Sec. \ref{rev:MR} for more details).
%\arc{Zhichuang can you comment on this given our new optimization?}
%Currently, TEE OS redoes the mapping of the TA’s pages on every world switch which results in high switch overhead. 

We thank the reviewer for the suggestion of a switchless approach and we will explore it for future direction (implementing it in ShadowNet would require some design changes). %Another possible optimization is to buffer the TA’s page mappings inside TEE which we consider to be feasible for industry usage. \todo
\\\\
\textcolor{red}{Concern 6. }\textit{In Figure 7, what obfuscation ratio is being used?}\\
\textcolor{blue}{Response 6. }The value of the obfuscation ratio $r$ is $1.2$, we have added this detail in the figure caption in the paper. \\\\
\textcolor{red}{Concern 7. }\textit{p.8 In bullet point 2, which inner and outer loops are being swapped?}\\\textcolor{blue}{Response 7.} This refers to the nested loops required for accessing multi-dimensional data.
\subsection*{Review B}
\noindent \textcolor{red}{Concern 1. }\textit{It is still unclear how many applications ShadowNet would be applicable to. The paper evaluated using relatively small and simple models. Given the spatial limitation due to the limited secure memory space in the TEE, it is still questionable if ShadowNet can deal with other apps that use more complicated and larger models.}\\
\textcolor{blue}{Response 1. }  We have added evaluations results for \textit{two} larger and complex models -- ResNet-404~\cite{he2016deep} and  YOLOv4-tiny~\cite{YOLOPaper} in Sec. \ref{sec:eval}. Additionally, we have analyzed the spatial overhead of ShadowNet and added a discussion on assessing how large a model can ShadowNet support. See our response to Concern 1 in Sec. \ref{rev:MR} of the revision letter for more details. 
%The amount of TEE memory required for running the ShadowNet transformed model can be estimated by the size of the weights that need to be stored inside the TEE (see ``Other" in the table above) which depends on the following two factors. First, it depends on the size of the transformed convolutional layers' weights which can be computed from shapes of the convolutional layers and the obfuscation ratio. Second, it depends on the weights of the mask layers which can be computed from the input and output shape of each layer. %As shown in Table \ref{tab:sd-size}, even though the original model can be big, the weights need to be stored inside TEE can be small (e.g., MiniVGG) or big (e.g., MobileNets). 
%Note that the actual runtime memory allocation required by ShadowNet is lesser due to our optimized memory allocation (Sec. \ref{sec:implementation:opt}).  We have added this discussion in Sec. \ref{sec:discussion}.
%For example, for MobileNet, the weights of the mask layers has a size of $37$MB which takes around $200$ms to be updated. For ResNet-$44$, the mask size is $3.3$MB which takes $18$ms to be updated. 
\\\\
\textcolor{red}{Concern 2. }\textit{Similarly, while the paper says that it can handle model layers of different types, such as LSTM, the authors do not evaluate any models that use them. If the paper provides a small example of it working for object recognition, audio recognition, etc., it will make the paper more convincing.}\\
\textcolor{blue}{Response 2. }We have added evaluation results for YOLOv4-tiny in Sec. \ref{sec:eval} which is the state-of-the-art object detection model that is more complex than a regular CNN. See our response to Concern 1 in Sec. \ref{rev:MR} of this revision letter for more details. 

LSTM's are the state-of-the-art models used for speech recognition. We have provided an illustration of ShadowNet's support for LSTMs in Sec. \ref{sec:discussion}. See our response for Concern 5 in Sec. \ref{rev:MR} of this revision letter for more details. 
\\\\\textcolor{red}{Concern 3. }\textit{The authors should utilize the Design section to provide the unique design consideration of ShadowNet rather than describing general concepts of CNN and DNN. Furthermore, the overall structure and organization of this paper would need to be reviewed and improved.}\\
\textcolor{blue}{Response 3. }We have rewritten the design section (Sec. \ref{sec:scheme}) as follows. We have moved all the discussion regarding general concepts of CNN to the background section (Sec. \ref{sec:background:CNN}). All the discussion in Sec. \ref{sec:scheme} now corresponds to ShadowNet specific design choices.

Additionally, we have included the following discussion on how ShadowNet's design addresses the challenges of mobile TEE (outlined in Sec. \ref{sec:challenges}). First, ShadowNet tackles the challenge of limited TEE memory by running only a subset of layers of the model inside the TEE. Specifically, it leaves the resource-heavy convolutional layers outside TEE.  Moreover, we propose design optimizations in Sec. \ref{sec:scheme_opt} which further reduce ShadowNet's computational load. In addition, we propose several implementation optimizations for reducing its memory consumption (see Sec. \ref{sec:implementation:opt} for details). Second, our design of the transformations provides a formal security guarantee (Thm.~\ref{thm:1}). Consequently, ShadowNet allows efficient outsourcing of the linear layers to the accelerators without compromising on security. Third, the new operations introduced by ShadowNet (for masking and linear tranformations) are relatively simple. As a result, ShadowNet's implementation adds only 2100 LOC into the TCB thereby overcoming the challenge of limited TCB size (see Sec. \ref{sec:implementation} for details). Note that TensorFlow Lite has tens of thousands of lines of code and porting it as a whole inside the TEE would require a much larger TCB. ShadowNet, by design, keeps it outside the TCB, thereby allowing a user to enjoy its rich functionality in a secure fashion with a small TCB.\\\\
\textcolor{red}{Concern 4. }\textit{The title of this paper feels a bit overclaiming.} \\
\textcolor{blue}{Response 4. }We have changed the title to ``ShadowNet: A Secure and Efficient On-device Model Inference System for Convolutational Neural Networks". 
\\\\ 
%\textcolor{red}{Concern 2. }\textit{An increase in inference time from 15 ms to 468 ms is stated to be tolerable in the introduction.}\\
%\textcolor{blue}{Response 2. } We have clarified throughtout the paper that this is a factual error -  the correct result is that ShadowNet incurs an overhead of 468ms (3X), 76ms (2.93X) and 15ms (1.88X) for MobileNets, ResNet-44 and MiniVGG, respectively. \\\\
\textcolor{red}{Concern 5. }\textit{There are logical flaws in comparing the proposed system to cryptographic-based systems (as ShadowNet is not cryptographic) and instead should be compared to other systems similar. }\\
\textcolor{blue}{Response 5. } The purpose of comparing it against end-to-end cryptographic models is to highlight the immense gain in performance we can achieve from a design like ShadowNet without sacrificing on a formal security guarantee. That being said, ShadowNet does rely on very light-weight crypto -- specifically, the mask layer is equivalent to one-time pad encryption~\cite{doi:10.1080/0161-119691885040} and refreshing the masks is the main source of overhead caused by ShadowNet.
\par Although there are multiple existing approaches for ML model protection, direct comparison with them is not suitable due to the following reasons.

\noindent\textbf{TensorScone}~\cite{kunkel2019tensorscone}. \begin{itemize} \item It is only evaluated on Inceptionv4 and has a 3.1$\times$ overhead with 330MB memory consumption -- these overheads are significantly higher than that of ShadowNet. 
\item It is designed for a cloud environment. On the other hand, ShadowNet is aimed at a mobile environment which is much more resource constrained.
\end{itemize}
\textbf{Slalom}~\cite{tramer2018slalom}.\begin{itemize}\item Unlike ShadowNet, Slalom does not protect model privacy.
\end{itemize}
\textbf{OMG}~\cite{bayerl2020offline}.\begin{itemize}
\item The original paper just presents a proof-of-concept implementation for OMG that cannot be directly integrated with existing mobile apps (unlike ShadowNet). 
\item Additionally, it is evaluated only on a single voice recognition model.
\item OMG is based on the Sanctuary enclave \cite{brasser2019sanctuary} which runs the user application along with the OS in an isolated environment. For model inference, the unmodified model is run inside the Sanctuary enclave. Consequently, the threat model is different as OMG requires the whole software stack including the OS, libraries and the application inside Sanctuary to be trusted. ShadowNet, on the other hand, relies only on a secure TEE-OS and TA which is a much more relaxed trust assumption.
\end{itemize}
\textbf{Graviton}~\cite{volos2018graviton}.\begin{itemize}\item
It requires hardware changes to the GPU which is not commercially available. \end{itemize}
The above discussion is included in Table \ref{tab:compare_works} and Sec. \ref{sec:related_work}.
\\\\
\textcolor{red}{Concern 6. }\textit{It is stated multiple times that linear layers are handled by the TEE. But at other times like in the prototype section, it is said that linear layers are only handled by the normal world, so not TEE?}\\
\textcolor{blue}{Response 6. } The core idea of ShadowNet is to outsource the heavy linear layers of the model to the untrusted hardware accelerators -- only non-linear layers are handled inside the TEE (Sec. \ref{sec:overview:sol}). We have thoroughly checked the paper to make sure there are no sentences stating otherwise.
\\\\\textcolor{red}{Concern 7. }\textit{...certain tradeoffs are not considered (r vs latency for example)}
\\
\textcolor{blue}{Response 7. } Fig. \ref{fig:obf_ratio} reports the relevant results. Specifically, we plot the change in model accuracy, model size (regularized) and model inference time (regularized) with varying obfuscation ratio, $r$.
\\\\\textcolor{red}{Concern 8. }\textit{Equation 4 unclear, is not given a definition anywhere. It seems to be an identity matrix with different values of lambda along the diagonal but once again this is unclear.}\\\textcolor{blue}{Response 8. } $\Lambda$ is a diagonal matrix where the diagonal elements $\lambda_i \in \F, i \in [n]$ are random scalars. We have added this detail in Sec. \ref{sec:transform}. \\\\
\textcolor{red}{Concern 9. }\textit{Citations for model choices would be appreciated as MiniVGG has no references besides the authors’ own paper when looking this up. The same applies to the "MobileNets", which ones did the authors use?}\\\textcolor{blue}{Response 9. }The citations for MiniVGG and MobileNets is \cite{simonyan2014very} (code \cite{minivggcode}) and \cite{howard2017mobilenets} (code \cite{Mobilenets_Code}), respectively.
\begin{comment}\textit{Given the spatial limitation due to the limited secure memory space in the TEE, it is still questionable if ShadowNet can deal with other apps that use more complicated and larger models.
The statement "a recent large scale study [SSLM21] shows that currently there exists thousands of apps that use on-device machine learning where ShadowNet is applicable." does not consider this spatial (model size) limitation.}
\\
\textcolor{blue}{Response 4. } In general, the amount of TEE memory required for running the ShadowNet transformed model can be estimated by the size of the weights that need to be stored inside the TEE (see ``Other" in Table \ref{tab:sd-size}). The size of the ShadowNet transformed model depends on two factors. First, it depends on the size of the transformed convolutional layers' weights which can be computed from the obfuscation ratio. Second, it depends on the weights of the mask layers which can be computed from the input and output shape of each layer. %As shown in Table \ref{tab:sd-size}, even though the original model can be big, the weights need to be stored inside TEE can be small (e.g., MiniVGG) or big (e.g., MobileNets). 
Thus, whether ShadowNet can support a given model can be checked by estimating the requisite TEE memory as discussed above. 
Note that the actual runtime memory allocation required by ShadowNet is lesser due to our optimized memory allocation as discussed in Sec. \ref{sec:ca-ta}. We have added this discussion in Sec. \ref{sec:eval}.\\\\
\end{comment}
%\noindent\textcolor{red}{Concern 5. }\textit{The authors should utilize the Design section to provide the unique design consideration of ShadowNet rather than describing general concepts of CNN and DNN.}\\\textcolor{blue}{Response 5. }
\\\\\textcolor{red}{Concern 10. }\textit{ First, I appreciate the additional explanation on proofs and it makes sense. If these detailed clarifications are provided in the paper, it would be helpful for readers to understand your design consideration.}\\
\textcolor{blue}{Response 10. } We are glad that our response helped. We have added the details in Sec. \ref{sec:sec_ana}. \\\\
\textcolor{red}{Concern 11. }\textit{ShadowNet assumes that the weights of linear layers remain unchanged, this assumption might limit the use case of ShadowNet given the recent trend that keeps refining the model.}
\\
\textcolor{blue}{Response 11. } We can apply ShadowNet as long as the model does not change its weights after every round of model inference. Specifically, ShadowNet’s weight conversion step can be integrated into the intermittent model update process.
\\\\
\textcolor{red}{Concern 12. } \textit{Writing needs to be redone for multiple sections.}\\
\textcolor{blue}{Response 12. }We have done a thorough pass on the paper to improve the writing. We have added all the missing citations.

\subsection{Review C}\label{rev:C}
\noindent \textcolor{red}{Concern 1.} \textit{Report the consistency. When you protect more layers, you may need to record the changes of consistency.}
\\
\textcolor{blue}{Response 1.} We have included the consistency numbers in Fig. \ref{fig:accuracy} in Sec. \ref{sec:eval}. See our response to Concern 3 in Sec. \ref{rev:MR} of the revision letter for more details.
\\\\\noindent \textcolor{red}{Concern 2.} \textit{Improve the accuracy of the models. You could refer to state-of-the-art to check the accuracy.}
\\
\textcolor{blue}{Response 2.} We have retrained all the models to match their corresponding state-of-the-art accuracies (Fig. \ref{fig:accuracy}, Sec. \ref{sec:eval}).
%\textcolor{white}{H}
%\textcolor{red}{Concern 1. }\textit{The overhead looks very high. As shown in Section VI-B, ShadowNet increases the model inference time from 15ms to 468ms, which is several times that of the original models. Such high overhead makes ShadowNet impractical to use in the real world. }\\
%\textcolor{blue}{Response 1. }
%We clarified in our rebuttal previously that this was a factual error. Additionally, after  --  the correct result is that ShadowNet incurs an overhead of 468ms (3X), 76ms (2.93X) and 15ms (1.88X) for MobileNets, ResNet-44 and MiniVGG, respectively. 
\\\\
\textcolor{red}{Concern 3. }\textit{Use more complicated and larger models.}
\\
\textcolor{blue}{Response 3. } We have added evaluations results for two larger and complex models -- ResNet-404~\cite{he2016deep} and  YOLOv4-tiny~\cite{YOLOPaper} in Sec. \ref{sec:eval}. See our response to Concern 1 in Sec. \ref{rev:MR} of the revision letter for more details.  \\\\
\textcolor{red}{Concern 4. }\textit{Evaluate the black-box attacks and provide more details. What kind of black-box attack are you using? How to choose the dataset for querying? What is the benefit of an attacker having cnn' compared to having no knowledge of the model? How many queries are needed to attack ShadowNet? Note that there is no limit to how many times an attacker can access the model.}
\\
\textcolor{blue}{Response 4.} We have added new evaluation results and details for the black-box attacks in Sec. \ref{sec:sec_ana}. See our response to Concern 4 in Sec. \ref{rev:MR} of the revision letter for more details. \\\\
\textcolor{red}{Concern 5. }\textit{The current overhead is high. It is better to further reduce the overhead.}
\\
\textcolor{blue}{Response 5. } We have proposed a new implementation optimization (Sec. \ref{sec:implementation:opt}) which has significantly improved our performance. The current overhead for ShadowNet varies from $0.6\times$ to $1.6\times$  as opposed to $1.8\times$ to $3\times$ (for our previous submission).  See our response to Concern 2 in Sec. \ref{rev:MR} of the revision letter for more details.
\\\\
\noindent\textcolor{red}{Concern 6. }\textit{Additionally, ShadowNet requires modifying Tensorflow-Lite, which also hinders real-world usage.}\\
\textcolor{blue}{Response 6. }The motivation of integrating ShadowNet into Tensorflow-Lite is two fold. First, it shows that it is feasible to apply ShadowNet on a mainstream on-device model inference platform.
Second, we make it extremely easy for Tensorflow-Lite users to adopt ShadowNet by simply updating the Tensorflow-lite library with our ShadowNet patch. This introduces no changes to the application logic, i.e., the model loading/inference interface remains the same as that of standard Tensorflow-Lite. Thus, our design of ShadowNet in fact makes it easier for real-world usage. We have included the details in Sec. \ref{sec:TF}.\\\\
\noindent\textcolor{red}{Concern 7. }\textit{Moreover, the authors should report the masks when assessing consistency. Different masks affect the results at different levels. A strong mask will protect the model better, but has a greater impact on accuracy.}\\
\textcolor{blue}{Response 7. } After quantization, every mask protects the model equally well since this is essentially equivalent to one-time pad encryption \cite{KatzLindell}. Additionally, the masks do not have a disparate effect on the model accuracy.\\\\ 
\textcolor{red}{Concern 8. }\textit{ ShadowNet increases the model inference time from 15ms to 468ms, which is several times that of the original model.}
\\
\textcolor{blue}{Response 8. } We clarified in our rebuttal that this statement was a factual error -- in our previous submission ShadowNet incurred an overhead of 468ms (3X), 76ms (2.93X) and 15ms (1.8X) for MobileNet, ResNet-44 and MiniVGG, respectively. As mentioned earlier, we have proposed a new optimization (Sec. \ref{sec:implementation:opt}) which has significantly improved our performance. The current overhead for ShadowNet for this \textit{revised submission} varies from $0.6\times$ to $1.6\times$  as opposed to $1.8\times$ to $3\times$ (for our previous submission).  See our response to Concern 2 in Sec. \ref{rev:MR} of the revision letter for more details.
\\\\\textcolor{red}{Concern 9. }\textit{... missing some details, like quantization parameters (e.g., prime p)...}\\
\textcolor{blue}{Response 9. } We use the same parameters as Slalom, namely a field $\mathbb{Z}_p$ for prime $p=2^{24}-3$ and fixed-point representation $l=8$. We have included the details in Sec. \ref{sec:efficiency}.
\\\\
\textcolor{red}{Concern 10. }\textit{The open-source repository is not accessible. }\\
\textcolor{blue}{Response 10. }We anonymized the link to comply with the anonymity requirements of the double blind review process since the repository might leak our identities. We will make the link public upon publication.
\subsection{Review D}
\noindent\textcolor{red}{Concern 1. }\textit{Evaluate and discuss in which usage scenarios running the model entirely inside the TEE is not feasible, and, consequently, ShadowNet can be useful.}
\\\textcolor{blue}{Response 1. } There are several challenges in running the unmodified model inside the TEE. First, standard model inference (outside the TEE) is memory intensive. For instance, convolution operations are expensive as they require resizing of the dimensions of the matrices. Additionally, buffers are allocated dynamically to store the intermediate results for the output of each layer.  Our memory profiling shows that running the unmodified model inference requires dynamically allocating at least 44MB for MiniVGG, 10MB for ResNet-44, 61MB for MobileNet, 54MB for ResNet-404 and 72MB for YOLOv4-tiny. Also note that the secure OS inside the TEE reserves $>$4MB memory for its usage. Hence given the TEE memory limit of $64$ MB for our evaluation board, it is not feasible to run the entire model inference task inside the TEE. ShadowNet, on the other hand, only requires 4MB for MiniVGG, 5MB for ResNet-44, 48MB for MobileNet, $34$MB for ResNet-404 and $37$MB for YOLOv4-tiny, thereby requiring a much smaller secure memory size. 

Second, running unmodified models inside the TEE would require a significant engineering effort. TensorFlow Lite needs to be ported into the TEE for the convolutional layers and matrix operations which rely on certain mathematical libraries (in C++) for efficiency. This entails a significant engineering effort since currently Arm OP-TEE OS does not support C++ and its corresponding computing libraries.  

Third, the limited size of the TCB presents additional challenges. A core focus of ShadowNet's design and implementation optimizations was to make it work with a small TCB -- its TA adds only 2100 LOC inside the TEE. Specifically, the new operations introduced by ShadowNet (LinearTransform, AddMask, ShuffleChannel) add $<$200 LOC into TCB as they are relatively simple operations.  On the other hand, TensorFlow Lite has tens of thousands lines of code and porting it as a whole inside TEE would require a much larger TCB. ShadowNet, by design, keeps it outside the TCB, thereby allowing a user to enjoy its rich functionality in a secure manner with a small TCB. Additionally, note that the extra code added for model conversion is used offline by the model vendor and is not deployed on the device. Hence, this does not increase the device TCB size. 

Last, we will lose access to hardware accelerators if we run the unmodified model inside the TEE.We have included the discussion in Secs.  \ref{sec:scheme_opt}, \ref{sec:implementation} and \ref{sec:discussion}. \\\\
\textcolor{red}{Concern 2. }\textit{Elaborate on how to set the ``obfuscation ratio" parameter in different real-world scenarios.}
\\
\textcolor{blue}{Response 2. }The obfuscation ratio $r$ is essentially a trade-off between the security guarantee (size of feasible sets, $\mathcal{F}(\hat{W})$, for model weights) and performance. The exact size of feasible sets can be analytically computed (see App. \ref{app:sec_ana}). Fig. \ref{fig:obf_ratio} shows ShadowNet’s performance with varying values of $r$. Based on this, we set $r=1.2$ for our experimental setup since this was the sweet spot. Specifically, even with $n=16$ (the smallest value of $n$ for our evaluation) and field $\mathbb{F}=\mathbb{Z}_p$
  for $p=2^{24}-3$, the size of the feasible set, $|\mathcal{F}(\hat{W})|$, is of the order of $2^{268}$ which is sufficient for security. We have included this discussion in Sec. \ref{sec:sec_ana}.
\\\\
\textcolor{red}{Concern 3. }\textit{What is the cause of the small (less than $1\%$) model prediction accuracy loss?}\\\textcolor{blue}{Response 3. }This loss occurs due to numerical errors of the quantization layer. The quantization is required for providing a formal security guarantee. We have included this explanation in Sec. \ref{sec:correctness} \\\\
\textcolor{red}{Concern 4. }\textit{How do the authors envision the model being loaded into the TEE? If the model is downloaded from a remote endpoint, some form of TEE attestation is required.}\\
\textcolor{blue}{Response 4. }ShadowNet’s design assumes that TEE is secure (just like prior work Slalom~\cite{tramer2018slalom}). Hence, for loading the model into TEE all standard attestation techniques apply (such as, loading an encrypted model and decrypting it inside the TEE) and this is orthogonal to our design. We have included this detail in Sec. \ref{sec:threat}.
\end{document}


==> demotext.tex <==
%-------------------------------------------------------------------------------
\section{Footnotes, Verbatim, and Citations}
%-------------------------------------------------------------------------------

Footnotes should be places after punctuation characters, without any
spaces between said characters and footnotes, like so.%
\footnote{Remember that USENIX format stopped using endnotes and is
  now using regular footnotes.} And some embedded literal code may
look as follows.

\begin{verbatim}
int main(int argc, char *argv[]) 
{
    return 0;
}
\end{verbatim}

Now we're going to cite somebody. Watch for the cite tag. Here it
comes. Arpachi-Dusseau and Arpachi-Dusseau co-authored an excellent OS
book, which is also really funny~\cite{arpachiDusseau18:osbook}, and
Waldspurger got into the SIGOPS hall-of-fame due to his seminal paper
about resource management in the ESX hypervisor~\cite{waldspurger02}.

The tilde character (\~{}) in the tex source means a non-breaking
space. This way, your reference will always be attached to the word
that preceded it, instead of going to the next line.

And the 'cite' package sorts your citations by their numerical order
of the corresponding references at the end of the paper, ridding you
from the need to notice that, e.g, ``Waldspurger'' appears after
``Arpachi-Dusseau'' when sorting references
alphabetically~\cite{waldspurger02,arpachiDusseau18:osbook}. 

It'd be nice and thoughtful of you to include a suitable link in each
and every bibtex entry that you use in your submission, to allow
reviewers (and other readers) to easily get to the cited work, as is
done in all entries found in the References section of this document.

Now we're going take a look at Section~\ref{sec:figs}, but not before
observing that refs to sections and citations and such are colored and
clickable in the PDF because of the packages we've included.

%-------------------------------------------------------------------------------
\section{Floating Figures and Lists}
\label{sec:figs}
%-------------------------------------------------------------------------------


%---------------------------
\begin{figure}
\begin{center}
\begin{tikzpicture}
  \draw[thin,gray!40] (-2,-2) grid (2,2);
  \draw[<->] (-2,0)--(2,0) node[right]{$x$};
  \draw[<->] (0,-2)--(0,2) node[above]{$y$};
  \draw[line width=2pt,blue,-stealth](0,0)--(1,1)
        node[anchor=south west]{$\boldsymbol{u}$};
  \draw[line width=2pt,red,-stealth](0,0)--(-1,-1)
        node[anchor=north east]{$\boldsymbol{-u}$};
\end{tikzpicture}
\end{center}
\caption{\label{fig:vectors} Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. }
\end{figure}
%% %---------------------------


Here's a typical reference to a floating figure:
Figure~\ref{fig:vectors}. Floats should usually be placed where latex
wants then. Figure\ref{fig:vectors} is centered, and has a caption
that instructs you to make sure that the size of the text within the
figures that you use is as big as (or bigger than) the size of the
text in the caption of the figures. Please do. Really.

In our case, we've explicitly drawn the figure inlined in latex, to
allow this tex file to cleanly compile. But usually, your figures will
reside in some file.pdf, and you'd include them in your document
with, say, \textbackslash{}includegraphics.

Lists are sometimes quite handy. If you want to itemize things, feel
free:

\begin{description}
  
\item[fread] a function that reads from a \texttt{stream} into the
  array \texttt{ptr} at most \texttt{nobj} objects of size
  \texttt{size}, returning returns the number of objects read.

\item[Fred] a person's name, e.g., there once was a dude named Fred
  who separated usenix.sty from this file to allow for easy
  inclusion.
\end{description}

\noindent
The noindent at the start of this paragraph in its tex version makes
it clear that it's a continuation of the preceding paragraph, as
opposed to a new paragraph in its own right.


\subsection{LaTeX-ing Your TeX File}
%-----------------------------------

People often use \texttt{pdflatex} these days for creating pdf-s from
tex files via the shell. And \texttt{bibtex}, of course. Works for us.

%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

The USENIX latex style is old and very tired, which is why
there's no \textbackslash{}acks command for you to use when
acknowledging. Sorry.

%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.



==> glossary.tex <==
\subsection{Glossary}
\point{Convolutional Layer}
A convolutional layer contains a set of filters whose parameters need to be learned. 
The height and weight of the filters are smaller than those of the input volume. 
Each filter is convolved with the input volume to compute an activation map made of neurons. 
In other words, the filter is slid across the width and height of the input and the dot products 
between the input and filter are computed at every spatial position. The output volume of 
the convolutional layer is obtained by stacking the activation maps of all filters along the depth dimension.

We also refer to the convolutional layer as the standard convolutional layer, so as to differentiate it
from other variants of convolutional layers.
\textbf{Conv} is used in the paper to represent the standard convolutional layer.

Mathematically speaking, the convolution operation on a given image $I$ with filter $K$
can be described as below, where $H$, $W$, $C$ represents the height, width and depth of
the filter $K$. The output of the convolution is a two-dimensional matrix. 

\begin{equation}
    Conv(I, K)_{x,y} =  \sum_{i=1}^{H}\sum_{j=1}^{W}\sum_{k=1}^{C}K_{i, j, k}I_{x+i-1, y+j-1, k}
\end{equation}

\point{Pointwise Convolutional Layer}
Pointwise Convolution is a type of convolution that uses a 1x1 kernel: a kernel that 
iterates through every single point. This kernel has a depth of however many channels 
the input image has. It can be used in conjunction with depthwise convolutions to 
produce an efficient class of convolutions known as depthwise-separable convolutions.

\textbf{PWConv} is used in the paper to represent the pointwise convolutional layer.
Mathematically speaking, the pointwise convolution operation on a given image $I$ with filter $K$
can be described as below, where $C$ represents the depth of
the filter $K$. The output of the convolution is a two-dimensional matrix. 

\begin{equation}
    PWConv(I, K)_{x,y} =  \sum_{k=1}^{C}K_{i, j, k}I_{x, y, k}
\end{equation}


\point{Depthwise Convolutional Layer}
Depthwise Convolution is a type of convolution where we apply a single convolutional 
filter for each input channel. In the regular 2D convolution performed over multiple 
input channels, the filter is as deep as the input and lets us freely mix channels to 
generate each element in the output. In contrast, depthwise convolutions keep each 
channel separate.

\textbf{DWConv} is used in the paper to represent the pointwise convolutional layer.
For a given image $I$ and filter $F$, the depthwise convolution $DWConv$ on input channel $c$ can be described as below, 
where $H$, $W$ represents the height and width of the filter $F$. The output is a two-dimensional matrix. 

\begin{equation}
    DWConv(I^{(c)}, F)_{x,y} =  \sum_{i=1}^{H}\sum_{j=1}^{W}F_{i, j}I_{x+i-1, y+j-1}^{(c)}
\end{equation}


\point{Transformation Matrix}
For standard convolutional layer, we only need to transform the weights.
We use $W$ to represent the weights before transformation, and $T$ to represent
the weights after transformation. We also use $\Lambda$ to represent the transformation matrix,
and $B$ to represent the restoration matrix used in the TEE.

The transformation of the weights $W$:
\begin{equation}
                              T^T = W^T \cdot \Lambda 
\end{equation}

The restoration of the weights $W$:

\begin{equation}
                              W^T = T^T \cdot B 
\end{equation}

The relationship between of the transformation matrix $\Lambda$ and restoration matrix $B$:

\begin{equation}
                              B = \Lambda^{-1} 
\end{equation}

For depthwise convolutional layer, we need to transform both the weights and the input.
We also use $W$ to represent the weights before transformation, and $T$ to represent
the weights after transformation. We also use $\Lambda$ to represent the transformation matrix for
the weights, and $B$ to represent the restoration matrix used in the TEE.
We use $A$ to represent the transformation matrix for the input.

The relationship between the weight transformation matrix $\Lambda$ and input transformation
matrix $A$ can be summarized as follows: (i)both of them adopt the same shuffling sequence. In our example of
\textbf{Reverse Input Channels}, both
$\Lambda$ and $A$ reverse the sequence; (ii) the scalar for the channel in $A$ should be the reciprocal of
the scalar for the corresponding filter in $\Lambda$, like $\lambda_{1}$ in $\Lambda$ and $1/\lambda_{1}$ in $A$.
The relationship between $A$ and $\Lambda$ can be also described with the following equation, where $I$ is an identity matrix.

\begin{equation}
    A \cdot \Lambda ^ T = I
\end{equation}


==> observation.tex <==
\section{Parallax Design}
% overview : observation --> algorithm/idea --> examples(conv, matmul) 
% Demo CNN : a end-to-end design 

Parallax design is based on two observations: 1) linear layers takes up
over 90\% of the computation time of DNN's model inference, so we can focus 
on optimizing linear layers; 2) linear transformation can be applied on
model weights so that the linear operations on tranformed weights can be offloaded
to GPU without leaking original weights. Based on the above observations, 
the idea of Parallax can be summarized as follow:

\begin{itemize}
\item We split the model into two parts: linear layers and non-linear layers;
We apply linear transformation on weights of linear layers with a group secret
parameters, and out-source
the operations onto GPU;

\item We do non-linear operations within TEE, and re-apply inverted linear 
transformation on the results of out-sourced operations with secret parameters.
\end{itemize}

Linear transformation is at the core of Parallax design. As it transform the original
linear operations into another vector space like a parallel world, where 
the confidentiality and efficiency of model weights can be kept at the same time. 
We will use examples to show how it works for concrete operations. 


Linear transformation is built on top of two important algebraic properties
that convolution and matrix multication share: \texttt{Distributivity} and 
\texttt{Associativity with scalar multiplication}.

%With these two properties, we can apply linear transformation on the weights
%of linear operations to obfuscate the weights and 
%The key idea of Parallax
%is built on top these two algebraic properties and apply linear transformation
%on the weights of linear layers like Convolution layer and Fully Connected layer. 
%For deep learning, 
%convolution, matrix multication, which are suitable for optimized hardware
%accelerators like GPU, TPU and NPU. 
TBD


==> other.tex <==
\section{Evaluation}
% system building challenges and optimizations
% normal world 
% A. correctness verification
%    error introduced by masking layer 
%    error ratio introduced by obfuscation
% B. performance without tee
%    scheme optimization and tuning 
%    1. get rid of mask layers
%    2. apply scheme on half of the layers
%    3. obfuscation ratio impact 
% C. performance with tee
%    implementation optimization
%    1. fuse optimization layers
%    2. pre-allocate buffer for weights and output, rotating output buffer
%    3. no masking layer's impact, fit all weights in tee
\subsection{Correctness Verification}
\point{Masking Layer Errors}
\point{Linear Transformation Errors}
\subsection{Static Overhead}
\point{Model Convertion}
\point{Model Loading}
\subsection{End-to-end System Evaluation}
\point{TEE Emulated}
\point{TEE Involved}
\point{Optimization}
\subsection{Adoption Efforts}
\subsection{TCB Analysis}

\section{Discussion}
\subsection{Automating Model Transformation}
\subsection{GPU Optimization}
\subsection{Expanding TEE Memory}

